Online Restless Multi-Armed Bandits with Long-Term Fairness Constraints

Restless multi-armed bandits (RMAB) have been widely used to model sequential decision making problems with constraints. The decision maker (DM) aims to maximize the expected total reward over an infinite horizon under an "instantaneous activation constraint" that at most B arms can be activated at any decision epoch, where the state of each arm evolves stochastically according to a Markov decision process (MDP). However, this basic model fails to provide any fairness guarantee among arms. In this paper, we introduce RMAB-F, a new RMAB model with "long-term fairness constraints", where the objective now is to maximize the long term reward while a minimum long-term activation fraction for each arm must be satisfied. For the online RMAB-F setting (i.e., the underlying MDPs associated with each arm are unknown to the DM), we develop a novel reinforcement learning (RL) algorithm named Fair-UCRL. We prove that Fair-UCRL ensures probabilistic sublinear bounds on both the reward regret and the fairness violation regret. Compared with off-the-shelf RL methods, our Fair-UCRL is much more computationally efficient since it contains a novel exploitation that leverages a low-complexity index policy for making decisions. Experimental results further demonstrate the effectiveness of our Fair-UCRL.

==> index.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Index Policy with Fairness Guarantees}\label{sec:index}

%Many efforts have been focusing on developing low-complexity solutions, among which, Whittle index policy \citep{whittle1988restless} has been found to exhibit good performance for \rmab problems, and is near-optimal \citep{weber1990index,verloop2016asymptotically}.  However, finding the Whittle index is typically intractable \citep{nino2007dynamic} and the Whittle indices of many practical problems remain unknown except for a few special cases.  Exacerbating this challenge is the fact that there is no such Whittle index policy for \frmab, since Whittle index policy has only been well defined for maximizing the total reward~(\ref{eq:FRMAB-obj}) under the activation constraint~(\ref{eq:FRMAB-constraint1}), without taking the fairness constraint~(\ref{eq:FRMAB-constraint2}) into account, and hence provides no fairness guarantees among arms.  We overcome this difficulty by developing a new index policy, which we call \fair that is computationally efficient and probably optimal.  


Instead of directly solving \frmab in~(\ref{eq:FRMAB-obj})-(\ref{eq:FRMAB-constraint2}), we propose an index policy for \frmab when the transition kernel $P_n$ and the reward function $r_n,\forall n\in\cN$ are known to the DM.  This index policy not only guarantees fairness for each arm, but also is provably asymptotically optimal.  


In order to describe the index policy in Section~\ref{sec:index-policy}, we first introduce a so-called ``relaxed problem".  Specifically, we relax the instantaneous activation constraint~(\ref{eq:FRMAB-constraint1}) to be satisfied on average \citep{whittle1988restless}, which leads to the following ``relaxed \frmab" (\refrmab) problem: 
\begin{align}
  \textbf{\refrmab}:\max_{\pi}&\liminf_{T \rightarrow \infty} \frac{1}{T}\mathbb{E}\Bigg[ \sum_{t=1}^T \sum_{n=1}^N r_n(t) \Bigg] \displaybreak[0]\label{eq:relaxed-FRMAB}\\
    \text{subject to}& \limsup_{T \rightarrow \infty}\! \frac{1}{T} \mathbb{E}\Bigg[\!\sum_{t=1}^T\!\sum_{n=1}^N a_{n}(t)\! \Bigg]\!\!\leq\! B,\displaybreak[1] \label{eq:relaxed-FRMAB-constraint1} \\
    & \liminf_{T \rightarrow \infty}\! \frac{1}{T} \mathbb{E}\Bigg[\!\sum_{t=1}^T a_n(t)\!\Bigg]\!\!\geq\!\eta_n, \forall n. \label{eq:relaxed-FRMAB-constraint2} 
\end{align}
One can easily check that the optimal reward achieved by \refrmab in~(\ref{eq:relaxed-FRMAB})-(\ref{eq:relaxed-FRMAB-constraint2}) is an upper bound of that achieved by \frmab in~(\ref{eq:FRMAB-obj})-(\ref{eq:FRMAB-constraint2}) due to the relaxation.  More importantly, \refrmab can be equivalently reduced to a LP in occupancy measures \citep{altman1999constrained}. 


\begin{definition}
The occupancy measure $\Omega_{\pi}$ of a stationary policy $\pi$ for the infinite-horizon MDP is defined as the expected average number of visits to each state-action pair $(s,a)$, i.e.,
\begin{align}\label{eq:occupancy-measure}
    \Omega_\pi \!=\!\Bigg\{ \zeta_n(s,a)\!\triangleq\! \lim_{T\rightarrow \infty}\!\frac{1}{T} \mathbb{E}_\pi \Bigg[ \sum_{t=1}^T \mathds{1} (s_n(t)\!=\! s, a_n(t)\!=\! a)\Bigg] \Bigg\vert \forall n\in\cN, s\in \cS, a\in \cA \Bigg\},
\end{align}
which satisfies $\sum_{s\in\cS}\sum_{a\in\cA}\zeta_n(s,a)=1,\forall n\in\cN$, and hence $\zeta_n,\forall n\in\cN$ is a probability measure. 
\end{definition}


We now introduce the following LP via replacing all random variables in \refrmab in~(\ref{eq:relaxed-FRMAB})-(\ref{eq:relaxed-FRMAB-constraint2}) with the occupancy measure corresponding to each arm $n$ \citep{altman1999constrained}: 
\begin{align}
   \max_{\zeta_n\in\Omega_\pi}&  \sum_{n=1}^N \sum_{s\in\cS}\sum_{a\in\cA} \zeta_{n}(s,a) \bar{r}_n(s,a)\label{eq:lp-obj}\\
   \text{subject to}&\sum_{n=1}^N \sum_{s\in\cS} \zeta_{n}(s,1) \leq B,\label{eq:lp-constraint1} \\
   &\sum_{s\in\cS} \zeta_n(s,1) \geq \eta_n, \forall n \in\cN,\label{eq:lp-constraint2}  \\
   &\sum_{s^\prime\in\cS}\sum_{a\in\cA} \zeta_{n}(s,a)P(s^\prime|s,a)=\sum_{s^\prime\in\cS}\sum_{a^\prime\in\cA}\zeta_{n}(s^\prime,a^\prime)P_n(s|s^\prime,a^\prime), 
\forall n\in\cN,\label{eq:lp-constraint3} \\
   &\sum_{s\in\cS}\sum_{a\in\cA}\zeta_n(s,a)=1,\forall n\in\cN, \label{eq:lp-constraint4} 
   %&\zeta_{n}(s,a)\geq 0, \forall s \in \cS,a \in \cA. \label{eq:lp-constraint5} 
\end{align}
where~(\ref{eq:lp-constraint1}) and~(\ref{eq:lp-constraint2}) are restatements of~(\ref{eq:relaxed-FRMAB-constraint1}) and~(\ref{eq:relaxed-FRMAB-constraint2}), respectively;~(\ref{eq:lp-constraint3}) represents the fluid transition of occupancy measure; and~(\ref{eq:lp-constraint4}) holds since the occupancy measure is a probability measure. Thus the feasible set of LP~(\ref{eq:lp-obj})-(\ref{eq:lp-constraint4}) is non-empty. We denote the optimal solution to LP~(\ref{eq:lp-obj})-(\ref{eq:lp-constraint4}) as $\Omega_{\pi^*}=\{\zeta_n^*(s,a),\forall n\in\cN, s\in\cS, a\in\cA\}$, and the corresponding optimal value as $V^*:=\sum_{n=1}^N \sum_{s\in\cS}\sum_{a\in\cA} \zeta_{n}^*(s,a) r_n(s,a)$, which upper bounds the reward of \frmab in~(\ref{eq:FRMAB-obj})-(\ref{eq:FRMAB-constraint2}). 


\subsection{An Index based Policy}\label{sec:index-policy}
Unfortunately, the solution to LP~(\ref{eq:lp-obj})-(\ref{eq:lp-constraint4}) is not always feasible to \frmab in~(\ref{eq:FRMAB-obj})-(\ref{eq:FRMAB-constraint2}).  This is due to the fact that the activation constraint~(\ref{eq:FRMAB-constraint2}) of \frmab must be satisfied at all time, rather than in the average sense as in~(\ref{eq:lp-constraint1}).  Exacerbating the challenge is the fact that the average activation constraint~(\ref{eq:lp-constraint1}) and the fairness constraint~(\ref{eq:lp-constraint2}) may be violated severely during the decision epoch, resulting in poor policy performance.  To overcome these challenges, we next introduce an index policy for \frmab. 

%Specifically, we first construct a Markovian policy as follows: if the state of arm $n$ at time $t$ is $s_n(t)=s$, then $\omega_{n}^*$ chooses action $a$ with probability 
%\begin{align}
%\omega_{n}^*(s,a)=\frac{\zeta_{n}^*(s,a)}{\sum_{a\in\cA}\zeta_{n}^*(s, a)}.
%\end{align}


Specifically, we derive our index policy on top of the optimal solution $\Omega_{\pi^*}=\{\zeta_n^*(s,a),\forall n\in\cN, s\in\cS, a\in\cA\}$. Since $\cA=\{0,1\}$, i.e, an arm can be either active or passive at time $t$, we define the index assigned to arm $n$ in state $s_n(t)=s$ at time $t$ to be as
\begin{align}\label{eq:fair-index}
\omega_{n}^*(s):=\frac{\zeta_{n}^*(s,1)}{\zeta_{n}^*(s, 1)+\zeta_{n}^*(s, 0)}.
\end{align}
We call this \textit{the fair index} since $\omega_{n}^*(s)$ represents the probability of activating arm $n$ in state $s$ towards maximizing the total rewards while guarantees fairness for arm $n$ in \frmab  in~(\ref{eq:FRMAB-obj})-(\ref{eq:FRMAB-constraint2}).   To this end, we rank all arms according to their indices in~(\ref{eq:fair-index}) in a non-increasing order, and activate the set of $B$ highest indexed arms, denoted as $\cN(t)\subset\cN$ such that $\sum_{n\in\cN(t)} a_n^*(t)\leq B$. All remaining arms are kept passive at time $t$. We denote the resultant index-based policy as $\pi^*=\{\pi_n^*, n\in\cN\}$, and call it the \fair index policy. 

\begin{remark}\label{remark:index}
Unlike Whittle-based policies \citep{whittle1988restless,hodge2015asymptotic,glazebrook2011general,zou2021minimizing,killian2021q}, our \fair index policy does not require the indexability condition, which is often hard to establish when the transition kernel of the underlying MDP is convoluted \citep{nino2007dynamic}. Like Whittle policies, our \fair index policy is computationally efficient since it is merely based on solving an LP.  A line of works \citep{hu2017asymptotically,zayas2019asymptotically,zhang2021restless,xiong2022reinforcement} designed index policies without indexability requirement for finite-horizon \rmab, and hence cannot be directly applied to our infinite-horizon average-cost formulation for \frmab in~(\ref{eq:FRMAB-obj})-(\ref{eq:FRMAB-constraint2}).  Finally, none of the aforementioned index policies guarantees fairness among arms, this is because these policies are only been well defined for maximizing the total reward~(\ref{eq:FRMAB-obj}) under the activation constraint~(\ref{eq:FRMAB-constraint1}), without taking the fairness constraint~(\ref{eq:FRMAB-constraint2}) into account. 
\end{remark}


\subsection{Asymptotic Optimality} 
We show that the \fair index policy is asymptotically optimal in the same asymptotic regime as that in state-of-the-art \rmab literature \citep{whittle1988restless,weber1990index,verloop2016asymptotically}.  For abuse of notation, we denote the number of arms as $\rho N$, the activation constraint  as $\rho B$ and the fairness constraint as \red{$\rho \eta_n, \forall n$} in the asymptotic regime with $\rho\rightarrow \infty$.  In other words, we consider $N$ classes of arms and will be interested in this fluid-scaling process with parameter $\rho.$ Let $X_n^\rho(\pi^*, s, a, t)$ be the number of class-n arms at state $s$ taking action $a$ at time $t$ under the \fair index policy $\pi^*$.  Denote the long-term reward as $V_{\pi^*}^\rho=\liminf_{T\rightarrow\infty}\mathbb{E}_{\pi^*}\sum_{t=1}^T\sum_{n=1}^N\sum_{(s, a)}r_n(s,a)\frac{X_n^\rho(\pi^*, s, a, t)}{\rho}$.  Then our \fair index policy $\pi^*$ is asymptotically optimal if and only if $V_{\pi^*}^\rho\geq V_{\pi}^\rho, \forall \pi$.




\begin{definition}\label{def:global-attractor}
An equilibrium point $X^{\rho,*}/\rho$ under the \fair index policy $\pi^*$ is a global attractor for the process ${X^\rho(\pi^*;t)}/{\rho}$, if, for any initial point ${X^\rho(\pi^*;0)}/{\rho}$,
the process ${X^\rho(\pi^*;t)}/{\rho}$ converges to $X^{\rho,*}/\rho.$
\end{definition}

\begin{remark}\label{remark:global-attractor}
The global attractor indicates that all trajectories converge to $X^{\rho,*}$.  Though it may be difficult to establish analytically that a fixed point is a global attractor for the process \citep{verloop2016asymptotically}, such assumption has been widely made in \rmab literature \citep{weber1990index,hodge2015asymptotic,verloop2016asymptotically,zou2021minimizing,duran2018asymptotic}, and is only verified numerically.  Our experimental results in Section~\ref{sec:exp} show that such convergence indeed occurs for our \fair index policy $\pi^*$.
\end{remark}

\begin{theorem}\label{thm:asy-optimality}
 \fair index policy $\pi^*$ is asymptotically optimal under Definition~\ref{def:global-attractor}, i.e., $\lim_{\rho\rightarrow\infty} V_{\pi^*}^\rho-V_{\pi^{opt}}^\rho=0$. 
\end{theorem} 

















